VIAFormer: Voxel-Image Alignment Transformer for High-Fidelity Voxel Refinement

We propose VIAFormer, a Voxel-Image Alignment Transformer model designed for Multi-view Conditioned Voxel Refinement--the task of repairing incomplete noisy voxels using calibrated multi-view images as guidance. Its effectiveness stems from a synergistic design: an Image Index that provides explicit 3D spatial grounding for 2D image tokens, a Correctional Flow objective that learns a direct voxel-refinement trajectory, and a Hybrid Stream Transformer that enables robust cross-modal fusion. Experiments show that VIAFormer establishes a new state of the art in correcting both severe synthetic corruptions and realistic artifacts on the voxel shape obtained from powerful Vision Foundation Models. Beyond benchmarking, we demonstrate VIAFormer as a practical and reliable bridge in real-world 3D creation pipelines, paving the way for voxel-based methods to thrive in large-model, big-data wave.

==> sec/X_suppl_2.tex <==
\section{More Results}\label{sec:more_results}

To further demonstrate the robustness and versatility of our method, this section provides additional qualitative results. Fig.~\ref{fig:more_noised_results} and \ref{fig:more_vfm_results} showcase more refinement outcomes on synthetic and VFM-derived noise, respectively.

Furthermore, we conduct an experiment to evaluate the model's capacity for half-space completion. The model is tasked with inferring the missing half of a shape, given the VFM-estimated image index ($\text{pos}_{I,i}$), four corresponding camera views ($\{I_i\}_{i=1}^4$), and one half of the ground-truth voxel grid ($v_{gt}$). The results, shown in Fig.~\ref{fig:halfspace_results}, indicate that our model is capable of reconstructing the missing geometry based on these inputs.

\section{Model Architecture Details}\label{sec:model_arch_detail}

This section provides detailed diagrams for the model architectures discussed in Sec.~\ref{sec:method}. Fig.~\ref{fig:viaformer_arch} illustrates the complete architecture of our proposed \abbr model. For the ablation studies, Fig.~\ref{fig:trellis_model_arch} details the baseline models used for comparison: (a) the geometry-only 24-Layer Self-Attention model, and (b) the 24-Layer Cross-Attention model with its various conditioning adapters.
